Enchanting Program Specification Synthesis by Large Language Models using Static Analysis and Program Verification

Formal verification provides a rigorous and systematic approach to ensure the correctness and reliability of software systems. Yet, constructing specifications for the full proof relies on domain expertise and non-trivial manpower. In view of such needs, an automated approach for specification synthesis is desired. While existing automated approaches are limited in their versatility, i.e., they either focus only on synthesizing loop invariants for numerical programs, or are tailored for specific types of programs or invariants. Programs involving multiple complicated data types (e.g., arrays, pointers) and code structures (e.g., nested loops, function calls) are often beyond their capabilities. To help bridge this gap, we present AutoSpec, an automated approach to synthesize specifications for automated program verification. It overcomes the shortcomings of existing work in specification versatility, synthesizing satisfiable and adequate specifications for full proof. It is driven by static analysis and program verification, and is empowered by large language models (LLMs). AutoSpec addresses the practical challenges in three ways: (1) driving \name by static analysis and program verification, LLMs serve as generators to generate candidate specifications, (2) programs are decomposed to direct the attention of LLMs, and (3) candidate specifications are validated in each round to avoid error accumulation during the interaction with LLMs. In this way, AutoSpec can incrementally and iteratively generate satisfiable and adequate specifications. The evaluation shows its effectiveness and usefulness, as it outperforms existing works by successfully verifying 79% of programs through automatic specification synthesis, a significant improvement of 1.592x. It can also be successfully applied to verify the programs in a real-world X509-parser project.

==> Code/annotated.tex <==
#include <limits.h>

/* 1. FUNC CONTRACT */
void swap(int *a, int *b) {
    // omitted
}

/* 4. FUNC CONTRACT */
void bubbleSort(int *array, int n) {
    int i, j;
    /* 3. LOOP INVARIANT */
    for(i = n - 1; i > 0; i--) {
        /* 2. LOOP INVARIANT */  |\label{code:loop-2}|
        for(j = 0; j < i; j++) {
            if (array[j] > array[j+1]) {
                swap(&array[j], &array[j+1]);
            }
        }
    }
}

void main() {
    // omitted
    //@ assert \forall int i; 0 < i < 5 ==> array[i-1] <= array[i];
}

==> Code/case-spurious.tex <==
int main() {
  int x = -50, y;
  // |\ding{53}| Loop invariant by Code2Inv:   ( ( x <= -50 |$\mid \mid$| y > ( 0 - 0 ) ) && ( x == ( x + 0 ) ) ) |\label{line:code2inv}|
  // |\ding{52}| Ground truth loop invariant: (x < 0 |$\mid \mid$| y > 0)
  while( x < 0 ) {   
    x = x+y;
    y++;
  }
  //@ assert(y>0);
}

==> Code/case-study-1.tex <==
void swap(int *a, int *b) {
	int temp = *a;
	*a = *b;
	*b = temp;
}

void bubbleSort(int *array, int n) {
	if (n <= 0) return;
	int i, j;
	for (i = n - 1; i > 0; i--) {
		for (j = 0; j < i; j++) {
			if (array[j] > array[j+1]) {
				swap(&array[j], &array[j+1]);
			}
		}
	}
}

void main() {
	int array [N] = {10, 7, 9, ...};
	bubbleSort(array, N);
}


==> Code/code-temp.tex <==
#include <assert.h> // include the header file for assert

void swap(int *a, int *b) {
	int temp = *a;
	*a = *b;
	*b = temp;
}

void bubbleSort(int *array, int n) {
	if (n <= 0) return;
	int i, j;
	for (i = n - 1; i > 0; i--) {
		for (j = 0; j < i; j++) {
			if (array[j] > array[j+1]) {
				swap(&array[j], &array[j+1]);
			}
		}
	}
}

void main() {
	int array [N] = {10, 7, 9, ...};
	bubbleSort(array, N);
}


==> Code/code-temp2.tex <==
#include <assert.h> // include the header file for assert

void swap(int *a, int *b) { // use pointers as parameters to swap the values
	int temp = *a;
	*a = *b;
	*b = temp;
}

void bubbleSort(int *array, int n) {
	assert(array != NULL); // precondition: array is not null
	assert(n >= 0); // precondition: n is non-negative
	if (n <= 0) return; // base case
	int i, j;
	for (i = n - 1; i > 0; i--) {
		assert(0 <= i && i <= n-1); // loop invariant: i is between 0 and n-1
		for (int k = 0; k < i; k++) { // loop invariant: the elements of the array from index 0 to index i are sorted in ascending order
			assert(array[k] <= array[k+1]);
		}
		for (j = 0; j < i; j++) {
			assert(0 <= j && j <= i); // loop invariant: j is between 0 and i
			for (int k = 0; k < j; k++) { // loop invariant: the elements of the array from index 0 to index j are sorted in ascending order
				assert(array[k] <= array[k+1]);
			}
			for (int k = j+1; k < n; k++) { // loop invariant: the element at index j is less than or equal to all the elements from index j+1 to index n-1
				assert(array[j] <= array[k]);
			}
			if (array[j] > array[j+1]) {
				swap(&array[j], &array[j+1]);
			}
		}
	}
	for (int i = 0; i < n-1; i++) { // postcondition: array is sorted in ascending order
		assert(array[i] <= array[i+1]);
	}
}

void main() {
	int array [N] = {10, 7, 9, ...};
	bubbleSort(array, N);
}


==> Code/infill.tex <==
void bubbleSort(int *array, int n) {
    int i, j;
    for(i = n - 1; i > 0; i--) {
        /* @ >>> INFILL <<< */
        for(j = 0; j < i; j++) {
            if (array[j] > array[j+1]) {
                swap(&array[j], &array[j+1]);
            }
        }
    }
}

==> Code/source-code.tex <==
void swap(int *a, int *b) {
    int temp = *a;
    *a = *b;
    *b = temp;
}

void bubbleSort(int *array, int n) {
    if (n <= 0) return;
    int i, j;
    for(i = n - 1; i > 0; i--) {
        for(j = 0; j < i; j++) {
            if (array[j] > array[j+1]) {
                swap(&array[j], &array[j+1]);
            }
        }
    }
}

void main() {
    int array[5000] = {..., 5, 4, 3, 2, 1};
    bubbleSort(array, 5000);
    //@ assert \forall int i; 0 < i < 5000 ==> array[i-1] <= array[i];
}

==> Figure/Fig-cases.tex <==
\begin{figure} [t]
    \centering
    \vspace{-0ex}
    \includegraphics[width=0.75\linewidth]{Figure/cases.pdf}
    \setlength{\abovecaptionskip}{-0pt}
    \setlength{\belowcaptionskip}{-0pt}
    \caption{Case Studies}
    \label{fig:case}
\end{figure}

==> Figure/Fig-moti2.tex <==
% \begin{figure} [t]
%     \centering
%     \vspace{-0ex}
%     \includegraphics[width=0.7\linewidth]{Figure/moti2.pdf}
%     \setlength{\abovecaptionskip}{-0pt}
%     \setlength{\belowcaptionskip}{-0pt}
%     \caption{Dependency Graph for Queue with Generic Support}
%     \label{fig:moti2}
% \end{figure}

% \begin{listing}[ht]
% \inputminted[
% frame=lines,
% framesep=1mm,
% baselinestretch=1.0,
% fontsize=\footnotesize,
% linenos,
% xleftmargin=5.5ex,
% baselinestretch=1.0,
% ]{c}{../Code/dependency_graph.c}
% \caption{Dependency Graph for Queue with Generic Support}
% \label{fig:moti2}
% \end{listing}

\definecolor{stubbg}{HTML}{FCF3D5}
\begin{figure}[t]
	\lstinputlisting[
		language=c,
		morekeywords={var},
		caption={Annotated Intermediate File},
		label={fig:moti2},
		escapechar=|,
		linebackgroundcolor = {\ifnum \value{lstnumber} = 13 \color{stubbg} \fi},
		numbers=left
	]{../Code/annotated.tex}
\end{figure}

==> Figure/Fig-moti3.tex <==
% \begin{figure} [t]
%     \centering
%     \vspace{-0ex}
%     \includegraphics[width=0.7\linewidth]{Figure/moti3.pdf}
%     \setlength{\abovecaptionskip}{-0pt}
%     \setlength{\belowcaptionskip}{-0pt}
%     \caption{Dependency Graph for Queue with Generic Support}
%     \label{fig:moti3}
% \end{figure}


% \begin{listing}[ht]
% \inputminted[
% frame=lines,
% framesep=1mm,
% baselinestretch=1.0,
% fontsize=\footnotesize,
% linenos,
% xleftmargin=5.5ex,
% baselinestretch=1.0,
% ]{c}{../Code/infill.c}
% \caption{Infill template}
% \label{fig:moti3}
% \end{listing}

\definecolor{stubbg}{HTML}{FCF3D5}
\begin{figure}[t]
	\lstinputlisting[
		language=c,
		morekeywords={var},
		caption={Infill template},
		label={fig:moti3},
		escapechar=|,
		linebackgroundcolor = {\ifnum \value{lstnumber} = 4 \color{stubbg} \fi},
		numbers=left
	]{../Code/infill.tex}
\end{figure}

==> Figure/case-study-1.tex <==
\definecolor{stubbg}{HTML}{FCF3D5}
\begin{figure}[h]
	\lstinputlisting[
		language=c,
        basicstyle=\linespread{1.0}\tiny,
		morekeywords={var},
		caption={case 1},
		label={fig:case1},
		escapechar=|,
		numbers=left
	]{../Code/case-study-1.tex}
\end{figure}

==> Figure/case-study-2.tex <==
\definecolor{stubbg}{HTML}{FCF3D5}
\begin{figure}[h]
	\lstinputlisting[
		language=c,
        basicstyle=\linespread{1.0}\tiny,
		morekeywords={var},
		caption={case 2},
		label={fig:case2},
		escapechar=|,
		numbers=left
	]{../Code/case-study-2.tex}
\end{figure}

==> Figure/case-study-3.tex <==
\definecolor{stubbg}{HTML}{FCF3D5}
\begin{figure}[t]
	\lstinputlisting[
		language=c,
        basicstyle=\linespread{1.0}\tiny,
		morekeywords={var},
		caption={case 3},
		label={fig:case3},
		escapechar=|,
		numbers=left
	]{../Code/case-study-3.tex}
\end{figure}

==> Listing/Listing-case1.tex <==
\definecolor{stubbg}{HTML}{FCF3D5}
\begin{figure}[h!]
	\lstinputlisting[
		language=c,
        basicstyle=\linespread{1.0}\tiny,
		morekeywords={var},
        aboveskip=-10pt,
        belowskip=-0pt,
		%label={listing:case1},
		escapechar=|,
        captionpos=none,
		linebackgroundcolor = {\ifnum \value{lstnumber} > 2 \ifnum \value{lstnumber} < 5 \color{stubbg} \fi \fi},
		numbers=left
	]{../Code/case-spurious.tex}
    \label{listing:case1}
\end{figure}

==> Listing/listing-temp1.tex <==
\definecolor{stubbg}{HTML}{FCF3D5}
\begin{figure}[h!]
\label{listing:case1}
	\lstinputlisting[
		language=c,
		morekeywords={var},
            % aboveskip=-8pt,
            % belowskip=-10pt,
		label={listing:case1},
		escapechar=|,
            captionpos=none,
		% linebackgroundcolor = {\ifnum \value{lstnumber} > 2 \ifnum \value{lstnumber} < 5 \color{stubbg} \fi \fi},
		numbers=left
	]{../Code/code-temp.tex}
\end{figure}

==> Listing/listing-temp2.tex <==
\definecolor{stubbg}{HTML}{FCF3D5}
\begin{figure}[h!]
\label{listing:case1}
	\lstinputlisting[
		language=c,
		morekeywords={var},
            % aboveskip=-8pt,
            % belowskip=-10pt,
		label={listing:case1},
		escapechar=|,
            captionpos=none,
		% linebackgroundcolor = {\ifnum \value{lstnumber} > 2 \ifnum \value{lstnumber} < 5 \color{stubbg} \fi \fi},
		numbers=left
	]{../Code/code-temp2.tex}
\end{figure}

==> Table/backup.tex <==
\begin{table*}[t!]
\centering
\setlength{\abovecaptionskip}{-0pt}
\setlength{\belowcaptionskip}{-0pt}
\caption{\textbf{Effectiveness on Loop Invariants}. {\footnotesize SyGuS~\cite{SyGuS} benchmark contains 133 C programs with one loop structure. While OOPSLA-13~\cite{oopsla13} benchmark contains 46 C programs with one loop, multiple loops, and nested loop structures. This table elaborates partial results on three baselines (Pailt, Code2Inv, and CLN2INV) compared with \name in the number of successfully verified programs and the overhead in seconds.}}
\label{tab:rq2-133-46}
\renewcommand\arraystretch{0.91}
    \resizebox{0.95\linewidth}{!}{
\begin{tabular}{ll|crcccrcr||rrrr|crcrrcr}
\toprule
\multicolumn{10}{c||}{\cellcolor[HTML]{CBE0B8}\textbf{SyGuS~\cite{SyGuS} (133 C Programs with One Loop)}} & \multicolumn{10}{c}{\cellcolor[HTML]{D2E1F1}\textbf{OOPSLA-13~\cite{oopsla13} (46 C Programs with Various Loop Types)}} \\
\midrule
\multicolumn{2}{c|}{\textbf{Info}} & \multicolumn{2}{c}{\cellcolor[HTML]{EBCB8B}\textbf{\name}} & \multicolumn{2}{c}{\textbf{Pailt}} & \multicolumn{2}{c}{\textbf{Code2Inv}} & \multicolumn{2}{c||}{\textbf{CLN2Inv}} & \multicolumn{4}{c|}{\textbf{Info}} & \multicolumn{2}{c}{\cellcolor[HTML]{EBCB8B}\textbf{\name}} & \multicolumn{2}{c}{\textbf{Code2Inv}} & \multicolumn{2}{c}{\textbf{CLN2INV}}\\
\midrule
ID & LoC & Sucess & Time(s) & Success & Time(s) & Success & Time(s) & Success & Time & ID & LoC & Type & \begin{tabular}[c]{@{}l@{}}Loop\\ Num.\end{tabular} & Success & \begin{tabular}[c]{@{}c@{}}\textbf{Time(s)}\\ \textbf{mean $\pm$ std}\end{tabular} & Success & Time(s) & Success & Time(s)\\
\rowcolor{rowcolor}
1 & 29 & \ding{52} & 6.65 & \ding{53} & -- & \ding{52} & 4950.78 & \ding{52} & 4.32 & 1 & 23 & Linear & 1 & \ding{52} & $ 6.25 \pm 7.22 $ & \ding{52} & 337.8 & \ding{108} & --\\
2 & 20 & \ding{52} & 5.97 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 4.11 & 2 & 27 & Linear & 1 & \ding{52} & $ 7.17 \pm 7.38 $ & \ding{52} & 74.36 & \ding{108} & --\\
\rowcolor{rowcolor}
3 & 18 & \ding{53} & 36.24 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 0.22 & 3 & 22 & Linear & 1 & \ding{52} & $ 113.47 \pm 88.10 $ & \ding{52} & 46.22 & \ding{53} & --\\
4 & 13 & \ding{53} & 32.28 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 0.21 & 4 & 28 & Linear & 1 & \ding{52} & $ 6.04 \pm 7.64 $ & \ding{53} & -- & \ding{108} & --\\
\rowcolor{rowcolor}
5 & 17 & \ding{52} & 19.22 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 2.48 & 5 & 30 & Linear & 1 & \ding{52} & $ 8.59 \pm 9.80 $ & \ding{53} &  & \ding{108} & --\\
6 & 21 & \ding{53} & 142.95 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 1.7 & 6 & 31 & Linear & 1 & \ding{52} & $ 41.62 \pm 24.06 $ & \ding{53} & -- & \ding{53} & -- \\
\rowcolor{rowcolor}
7 & 17 & \ding{52} & 57.15 & \ding{53} & -- & \ding{52} & 128.03 & \ding{52} & 3.47 & 7 & 30 & Linear & 1 & \ding{52} & $ 12.66 \pm 15.12 $ & \ding{53} & -- & \ding{108} & --\\
8 & 15 & \ding{52} & 92.75 & \ding{53} & -- & \ding{52} & 72.74 & \ding{52} & 3.13 & 8 & 24 & Linear & 1 & \ding{52} & $ 3.40 \pm 3.25 $ & \ding{53} & -- & \ding{108} & --\\
\rowcolor{rowcolor}
9 & 25 & \ding{52} & 39.66 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 3.04 & 9 & 27 & Linear & 1 & \ding{53} & -- & \ding{53} & -- & \ding{53} & --\\
10 & 21 & \ding{53} & 295.83 & \ding{53} & -- & \ding{52} & 53.39 & \ding{52} & 3.14 & 10 & 26 & Linear & 1 & \ding{52} & $ 9.40 \pm 7.29 $ & \ding{53} & -- & \ding{108} & --\\
\rowcolor{rowcolor}
11 & 18 & \ding{52} & 77.48 & \ding{53} & -- & \ding{52} & 145.02 & \ding{52} & 3.33 & 11 & 26 & Linear & 1 & \ding{52} & $ 16.82 \pm 16.90 $ & \ding{53} & -- & \ding{53} & --\\
12 & 30 & \ding{52} & 106.137 & \ding{53} & -- & \ding{52} & 71.97 & \ding{52} & 3.37 & 12 & 25 & Linear & 1 & \ding{52} & $ 51.27 \pm 34.43 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
13 & 31 & \ding{52} & 240.24 & \ding{53} & -- & \ding{52} & 39.82 & \ding{52} & 3.07 & 13 & 25 & Linear & 1 & \ding{52} & $ 12.57 \pm 10.57 $ & \ding{53} & -- & \ding{108} & --\\
14 & 18 & \ding{52} & 79.59 & \ding{53} & -- & \ding{52} & 21.9 & \ding{52} & 3.23 & 14 & 29 & Linear & 1 & \ding{52} & $ 19.42 \pm 11.52 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
15 & 20 & \ding{52} & 13.66 & \ding{53} & -- & \ding{52} & 274.79 & \ding{52} & 2.43 & 15 & 37 & Linear & 1 & \ding{52} & $ 58.85 \pm 13.83 $ & \ding{53} & -- & \ding{108} & --\\
16 & 22 & \ding{52} & 30.31 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 6.16 & 16 & 37 & Linear & 1 & \ding{53} & -- & \ding{53} & -- & \ding{108} & --\\
\rowcolor{rowcolor}
17 & 15 & \ding{52} & 24.97 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 2.31 & 17 & 27 & Linear & 1 & \ding{52} & $ 4.80 \pm 3.62 $ & \ding{52} & 66.4 & \ding{53} & --\\
18 & 22 & \ding{52} & 23.7 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 6.47 & 18 & 24 & Linear & 1 & \ding{52} & $ 19.86 \pm 12.17 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
19 & 33 & \ding{52} & 21.41 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 2.47 & 19 & 23 & Linear & 1 & \ding{52} & $ 10.34 \pm 7.59 $ & \ding{53} & -- & \ding{108} & --\\
20 & 22 & \ding{52} & 16.59 & \ding{53} & -- & \ding{52} & 53.57 & \ding{52} & 9.78 & 20 & 25 & Linear & 1 & \ding{53} & -- & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
21 & 21 & \ding{52} & 18.46 & \ding{53} & -- & \ding{52} & 114.8 & \ding{52} & 2.43 & 21 & 24 & Linear & 1 & \ding{52} & $ 12.09 \pm 7.97 $ & \ding{53} & -- & \ding{108} & --\\
22 & 20 & \ding{52} & 18.26 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 9.03 & 22 & 22 & Linear & 1 & \ding{52} & $ 11.79 \pm 11.14 $ & \ding{52} & 29.96 & \ding{108} & --\\
\rowcolor{rowcolor}
23 & 32 & \ding{53} & 108.75 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 2.52 & 23 & 28 & Linear & 1 & \ding{52} & $ 32.71 \pm 24.14 $ & \ding{53} & -- & \ding{53} & --\\
24 & 29 & \ding{53} & 80.94 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 2.38 & 24 & 23 & Linear & 1 & \ding{52} & $ 12.84 \pm 7.20 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
25 & 20 & \ding{52} & 5.43 & \ding{53} & -- & \ding{52} & 16.97 & \ding{52} & 0.2 & 25 & 62 & Linear & 1 & \ding{52} & $ 6.64 \pm 4.62 $ & \ding{53} & -- & \ding{53} & --\\
26 & 33 & \ding{53} & 91.67 & \ding{53} & -- & \ding{53} & -- & \ding{53} & 0 & 26 & 32 & Linear & 1 & \ding{52} & $ 44.89 \pm 49.35 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
27 & 29 & \ding{53} & 86.25 & \ding{53} & -- & \ding{53} & -- & \ding{53} & 0 & 27 & 34 & Linear & 1 & \ding{53} & -- & \ding{53} & -- & \ding{53} & --\\
28 & 21 & \ding{53} & 103.25 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 2.2 & 28 & 26 & Linear & 1 & \ding{52} & $ 11.92 \pm 9.78 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
29 & 25 & \ding{52} & 2.9 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 1.78 & 29 & 35 & Linear & 1 & \ding{52} & $ 16.21 \pm 14.83 $ & \ding{53} & -- & \ding{53} & --\\
30 & 19 & \ding{52} & 3.45 & \ding{53} & -- & \ding{52} & 0.69 & \ding{52} & 0.21 & 30 & 29 & Linear & 1 & \ding{52} & $ 140.51 \pm 67.06 $ & \ding{53} & -- & \ding{108} & --\\
\rowcolor{rowcolor}
31 & 22 & \ding{53} & 67.36 & \ding{53} & -- & \ding{53} & -- & \ding{53} & 0 & 31 & 51 & Multiple & 4 & \ding{53} & -- & \ding{53} & -- & \ding{53} & --\\
32 & 25 & \ding{53} & 27.54 & \ding{53} & -- & \ding{53} & -- & \ding{53} & 0 & 32 & 36 & Multiple & 2 & \ding{52} & $ 71.74 \pm 60.13 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
33 & 20 & \ding{52} & 2.73 & \ding{53} & -- & \ding{52} & 189.06 & \ding{52} & 2.07 & 33 & 27 & Multiple & 2 & \ding{52} & $ 94.02 \pm 58.68 $ & \ding{52} & 26.97 & \ding{53} & --\\
34 & 24 & \ding{52} & 3.47 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 1.34 & 34 & 33 & Multiple & 2 & \ding{52} & $ 57.32 \pm 39.28 $ & \ding{53} & -- & \ding{108} & --\\
\rowcolor{rowcolor}
35 & 22 & \ding{52} & 4.75 & \ding{53} & -- & \ding{52} & 12.04 & \ding{52} & 0.13 & 35 & 27 & Nested & 3 & \ding{52} & $ 58.26 \pm 54.18 $ & \ding{53} & -- & \ding{108} & --\\
36 & 34 & \ding{52} & 4.618 & \ding{53} & -- & \ding{52} & 5.69 & \ding{52} & 0.12 & 36 & 30 & Nested & 2 & \ding{52} & $ 84.23 \pm 57.52 $ & \ding{52} & 17.42 & \ding{53} & --\\
\rowcolor{rowcolor}
37 & 30 & \ding{52} & 6.99 & \ding{53} & -- & \ding{52} & 0.72 & \ding{52} & 0.16 & 37 & 23 & Nested & 2 & \ding{53} & -- & \ding{52} & 0.26 & \ding{108} & --\\
38 & 16 & \ding{52} & 3.43 & \ding{53} & -- & \ding{52} & 0.25 & \ding{52} & 0.27 & 38 & 22 & Nested & 3 & \ding{52} & $ 105.28 \pm 60.01 $ & \ding{53} & -- & \ding{108} & --\\
\rowcolor{rowcolor}
39 & 29 & \ding{52} & 12.94 & \ding{53} & -- & \ding{52} & 0.57 & \ding{52} & 0.16 & 39 & 35 & Nested & 2 & \ding{52} & $ 96.50 \pm 68.99 $ & \ding{53} & -- & \ding{53} & --\\
40 & 18 & \ding{52} & 2.22 & \ding{53} & -- & \ding{52} & 0.84 & \ding{52} & 0.17 & 40 & 26 & Nested & 3 & \ding{52} & $ 139.88 \pm 92.53 $ & \ding{52} & 147.89 & \ding{53} & --\\
\rowcolor{rowcolor}
41 & 23 & \ding{52} & 3.29 & \ding{53} & -- & \ding{52} & 39 & \ding{52} & 0.25 & 41 & 30 & Nested & 2 & \ding{52} & $ 177.43 \pm 106.79 $ & \ding{53} & -- & \ding{53} & -- \\
42 & 21 & \ding{52} & 23.19 & \ding{53} & -- & \ding{52} & 0.67 & \ding{52} & 0.11 & 42 & 29 & Nested & 3 & \ding{52} & $ 228.71 \pm 218.43 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
43 & 24 & \ding{52} & 18.13 & \ding{53} & -- & \ding{52} & 3.14 & \ding{52} & 0.11 & 43 & 39 & Nested & 3 & \ding{53} & -- & \ding{53} & -- & \ding{53} & --\\
44 & 21 & \ding{52} & 4.08 & \ding{53} & -- & \ding{52} & 3.21 & \ding{52} & 0.12 & 44 & 61 & Nested & 4 & \ding{53} & -- & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
45 & 29 & \ding{52} & 34.85 & \ding{53} & -- & \ding{52} & 0.56 & \ding{52} & 0.13 & 45 & 46 & Nested & 3 & \ding{52} & $ 202.78 \pm 185.39 $ & \ding{53} & -- & \ding{53} & --\\
\multicolumn{2}{c|}{} & \multicolumn{8}{c||}{\cellcolor[HTML]{8FBCBB}88 more cases are omitted due to space limitation} & 46 & 24 & Nested & 3 & \ding{52} & $ 86.61 \pm 50.22 $ & \ding{53} & -- & \ding{108} & --\\
\midrule
Total &  & \textbf{114 / 133} &  & 0/133 &  & 73 / 133 & $ 248.01 \pm 982.23 $ & \textbf{124 / 133} & $ 2.1 \pm 2.32$ &  &  &  &  & \textbf{38 / 46} & $ 68.92 \pm 171.13 $  & 9 / 46 & $ 83.03 \pm 104.84 $ & 0 / 46 &\\
\bottomrule
\end{tabular}
}
%\vspace{-15pt}
\end{table*}

==> Table/rq2-133.tex <==
\begin{table*}[thb]
\centering
\setlength{\abovecaptionskip}{-0pt}
\setlength{\belowcaptionskip}{-0pt}
\caption{\textbf{Effectiveness on Linear Loop Invariant}. SyGuS~\cite{SyGuS13} benchmark contains 133 C programs with one loop structure. This table elaborates partial results on three baselines (Pailt, Code2Inv and CLN2INV) compared with \name in terms of the number of successfully verified programs and the overhead used in seconds.}
\label{tab:rq2-133}
\renewcommand\arraystretch{1.0}
    \resizebox{0.9\linewidth}{!}{
\begin{tabular}{ll|ccrrr|cr|cr|cr}
\toprule
\multicolumn{2}{c|}{Benchmark Info} & \multicolumn{5}{c|}{\name} & \multicolumn{2}{c|}{Pailt} & \multicolumn{2}{c|}{Code2Inv} & \multicolumn{2}{c}{CLN2Inv} \\ 
\midrule
ID & LoC & Success & \begin{tabular}[c]{@{}l@{}}Iterations\\ Max = 5\end{tabular} & \begin{tabular}[c]{@{}l@{}}Solved\\ time(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}LLMs Query\\  time (s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Tokens\\ Cost\end{tabular} & Success & Time(s) & Success & Time(s) & Success & Time(s) \\
1 & 29 & \ding{52} & 1 & 6.65 & 2.99 & 1472 & \ding{53} & - & \ding{52} & 4950.78 & \ding{52} & 4.32 \\
2 & 20 & \ding{52} & 1 & 5.97 & 3.35 & 1468 & \ding{53} & - & \ding{53} & - & \ding{52} & 4.11 \\
3 & 18 & \ding{53} & Max & 36.24 & 22.13 & 94.8 & \ding{53} & - & \ding{53} & - & \ding{52} & 0.22 \\
4 & 13 & \ding{53} & Max & 32.28 & 16.52 & 9324 & \ding{53} & - & \ding{53} & - & \ding{52} & 0.21 \\
5 & 17 & \ding{52} & 1 & 19.22 & 3.25 & 1471 & \ding{53} & - & \ding{53} & - & \ding{52} & 2.48 \\
6 & 21 & \ding{53} & Max & 142.95 & 19.53 & 9375 & \ding{53} & - & \ding{53} & - & \ding{52} & 1.70 \\
7 & 17 & \ding{52} & 2 & 57.15 & 7.26 & 3397 & \ding{53} & - & \ding{52} & 128.03 & \ding{52} & 3.47 \\
8 & 15 & \ding{52} & 2 & 92.75 & 10.45 & 3455 & \ding{53} & - & \ding{52} & 72.74 & \ding{52} & 3.13 \\
9 & 25 & \ding{52} & 1 & 39.66 & 3.86 & 1508 & \ding{53} & - & \ding{53} & - & \ding{52} & 3.04 \\
10 & 21 & \ding{53} & Max & 295.83 & 29.88 & 10044 & \ding{53} & - & \ding{52} &  & \ding{52} & 3.14 \\
11 & 18 & \ding{52} & 2 & 77.48 & 6.5 & 3446 & \ding{53} & - & \ding{52} & 145.02 & \ding{52} & 3.33 \\
12 & 30 & \ding{52} & 3 & 106.137 & 14.96 & 5520 & \ding{53} & - & \ding{52} & 71.97 & \ding{52} & 3.37 \\
13 & 31 & \ding{52} & 4 & 240.24 & 19.51 & 7227 & \ding{53} & - & \ding{52} & 39.82 & \ding{52} & 3.07 \\
14 & 18 & \ding{52} & 4 & 79.59 & 15.1 & 7315 & \ding{53} & - & \ding{52} & 21.9 & \ding{52} & 3.23 \\
15 & 20 & \ding{52} & 1 & 13.66 & 5.08 & 1451 & \ding{53} & - & \ding{52} & 274.79 & \ding{52} & 2.43 \\
16 & 22 & \ding{52} & 1 & 30.31 & 3.77 & 1458 & \ding{53} & - & \ding{53} & - & \ding{52} & 6.16 \\
17 & 15 & \ding{52} & 1 & 24.97 & 3.58 & 1496 & \ding{53} & - & \ding{53} & - & \ding{52} & 2.31 \\
18 & 22 & \ding{52} & 1 & 23.7 & 4.21 & 1474 & \ding{53} & - & \ding{53} & - & \ding{52} & 6.47 \\
19 & 33 & \ding{52} & 1 & 21.41 & 3.27 & 1463 & \ding{53} & - & \ding{53} & - & \ding{52} & 2.47 \\
20 & 22 & \ding{52} & 1 & 16.59 & 3.46 & 1523 & \ding{53} & - & \ding{52} & 53.57 & \ding{52} & 9.78 \\
21 & 21 & \ding{52} & 1 & 18.46 & 3.18 & 1456 & \ding{53} & - & \ding{52} & 114.8 & \ding{52} & 2.43 \\
22 & 20 & \ding{52} & 1 & 18.26 & 3.81 & 1462 & \ding{53} & - & \ding{53} & - & \ding{52} & 9.03 \\
23 & 32 & \ding{53} & Max & 108.75 & 20.41 & 7571 & \ding{53} & - & \ding{53} & - & \ding{52} & 2.52 \\
24 & 29 & \ding{53} & Max & 80.94 & 15.54 & 7770 & \ding{53} & - & \ding{53} & - & \ding{52} & 2.38 \\
25 & 20 & \ding{52} & 1 & 5.43 & 3.36 & 1339 & \ding{53} & - & \ding{52} & 16.97 & \ding{52} & 0.2 \\
26 & 33 & \ding{53} & Max & 91.67 & 22.97 & 8832 & \ding{53} & - & \ding{53} & - & \ding{53} & 0 \\
27 & 29 & \ding{53} & Max & 86.25 & 26.98 & 9367 & \ding{53} & - & \ding{53} & - & \ding{53} & 0 \\
28 & 21 & \ding{53} & Max & 103.25 & 13.76 & 8713 & \ding{53} & - & \ding{53} & - & \ding{52} & 2.2 \\
29 & 25 & \ding{52} & 1 & 2.9 & 2.72 & 1378 & \ding{53} & - & \ding{53} & - & \ding{52} & 1.78 \\
30 & 19 & \ding{52} & 1 & 3.45 & 2.48 & 1322 & \ding{53} & - & \ding{52} & 0.69 & \ding{52} & 0.21 \\
31 & 22 & \ding{53} & Max & 67.36 & 36.89 & 10510 & \ding{53} & - & \ding{53} & - & \ding{53} & 0 \\
32 & 25 & \ding{53} & Max & 27.54 & 14.65 & 8944 & \ding{53} & - & \ding{53} & - & \ding{53} & 0 \\
33 & 20 & \ding{52} & 1 & 2.73 & 2.08 & 1357 & \ding{53} & - & \ding{52} & 189.06 & \ding{52} & 2.07 \\
% 34 & 24 & \ding{52} & 1 & 3.47 & 4.29 & 1372 & \ding{53} & - & \ding{53} & - & \ding{52} & 1.34 \\
% 35 & 22 & \ding{52} & 1 & 4.75 & 3.22 & 1393 & \ding{53} & - & \ding{52} & 12.04 & \ding{52} & 0.13 \\
% 36 & 34 & \ding{52} & 1 & 4.618 & 3.63 & 1402 & \ding{53} & - & \ding{52} & 5.69 & \ding{52} & 0.12 \\
% 37 & 30 & \ding{52} & 1 & 6.99 & 2.9 & 1464 & \ding{53} & - & \ding{52} & 0.72 & \ding{52} & 0.16 \\
% 38 & 16 & \ding{52} & 1 & 3.43 & 3.01 & 1411 & \ding{53} & - & \ding{52} & 0.25 & \ding{52} & 0.27 \\
% 39 & 29 & \ding{52} & 1 & 12.94 & 2.36 & 1370 & \ding{53} & - & \ding{52} & 0.57 & \ding{52} & 0.16 \\
% 40 & 18 & \ding{52} & 1 & 2.22 & 2.19 & 1411 & \ding{53} & - & \ding{52} & 0.84 & \ding{52} & 0.17 \\
\midrule
\multicolumn{13}{c}{\color{teal} 100 more cases are omitted due to space limitation} \\
\midrule
Total &  & \textbf{114 / 133} &  &  &  &  & 0 / 133 &  & 73 / 133 &  & \textbf{124 / 133} & \\
\bottomrule
\end{tabular}
}
\end{table*}

==> Table/rq2-46-133.tex <==
\begin{table*}[t!]
\centering
\setlength{\abovecaptionskip}{-0pt}
\setlength{\belowcaptionskip}{-0pt}
\caption{\textbf{Effectiveness on Loop Invariants}. {\footnotesize SyGuS~\cite{SyGuS} benchmark contains 133 C programs with one loop structure. While OOPSLA-13~\cite{oopsla13} benchmark contains 46 C programs with one loop, multiple loops, and nested loop structures. This table elaborates partial results on three baselines (Pailt, Code2Inv, and CLN2INV) compared with \name in the number of successfully verified programs and the overhead in seconds.}}
\label{tab:rq2-133-46}
\renewcommand\arraystretch{1.1}
    \resizebox{0.95\linewidth}{!}{
\begin{tabular}{ll|crcccrcr||rrrr|crcrrcr}
\toprule
\multicolumn{10}{c||}{\cellcolor[HTML]{CBE0B8}\textbf{SyGuS~\cite{SyGuS} (133 C Programs with One Loop)}} & \multicolumn{10}{c}{\cellcolor[HTML]{D2E1F1}\textbf{OOPSLA-13~\cite{oopsla13} (46 C Programs with Various Loop Types)}} \\
\midrule
\multicolumn{2}{c|}{\textbf{Info}} & \multicolumn{2}{c}{\cellcolor[HTML]{EBCB8B}\textbf{\name}} & \multicolumn{2}{c}{\textbf{Pailt}} & \multicolumn{2}{c}{\textbf{Code2Inv}} & \multicolumn{2}{c||}{\textbf{CLN2Inv}} & \multicolumn{4}{c|}{\textbf{Info}} & \multicolumn{2}{c}{\cellcolor[HTML]{EBCB8B}\textbf{\name}} & \multicolumn{2}{c}{\textbf{Code2Inv}} & \multicolumn{2}{c}{\textbf{CLN2INV}}\\
\midrule
ID & LoC & Sucess & Time(s) & Success & Time(s) & Success & Time(s) & Success & Time & ID & LoC & Type & \begin{tabular}[c]{@{}l@{}}Loop\\ Num.\end{tabular} & Success & \begin{tabular}[c]{@{}c@{}}\textbf{Time(s)}\\ \textbf{mean $\pm$ std}\end{tabular} & Success & Time(s) & Success & Time(s)\\
\rowcolor{rowcolor}
1 & 29 & \ding{52} & 6.65 & \ding{53} & -- & \ding{52} & 4950.78 & \ding{52} & 4.32 & 1 & 23 & Linear & 1 & \ding{52} & $ 6.25 \pm 7.22 $ & \ding{52} & 337.8 & \ding{108} & --\\
2 & 20 & \ding{52} & 5.97 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 4.11 & 2 & 27 & Linear & 1 & \ding{52} & $ 7.17 \pm 7.38 $ & \ding{52} & 74.36 & \ding{108} & --\\
\rowcolor{rowcolor}
3 & 18 & \ding{53} & 36.24 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 0.22 & 3 & 22 & Linear & 1 & \ding{52} & $ 113.47 \pm 88.10 $ & \ding{52} & 46.22 & \ding{53} & --\\
4 & 13 & \ding{53} & 32.28 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 0.21 & 4 & 28 & Linear & 1 & \ding{52} & $ 6.04 \pm 7.64 $ & \ding{53} & -- & \ding{108} & --\\
\rowcolor{rowcolor}
5 & 17 & \ding{52} & 19.22 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 2.48 & 5 & 30 & Linear & 1 & \ding{52} & $ 8.59 \pm 9.80 $ & \ding{53} &  & \ding{108} & --\\
6 & 21 & \ding{53} & 142.95 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 1.7 & 6 & 31 & Linear & 1 & \ding{52} & $ 41.62 \pm 24.06 $ & \ding{53} & -- & \ding{53} & -- \\
\rowcolor{rowcolor}
7 & 17 & \ding{52} & 57.15 & \ding{53} & -- & \ding{52} & 128.03 & \ding{52} & 3.47 & 7 & 30 & Linear & 1 & \ding{52} & $ 12.66 \pm 15.12 $ & \ding{53} & -- & \ding{108} & --\\
8 & 15 & \ding{52} & 92.75 & \ding{53} & -- & \ding{52} & 72.74 & \ding{52} & 3.13 & 8 & 24 & Linear & 1 & \ding{52} & $ 3.40 \pm 3.25 $ & \ding{53} & -- & \ding{108} & --\\
\rowcolor{rowcolor}
9 & 25 & \ding{52} & 39.66 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 3.04 & 9 & 27 & Linear & 1 & \ding{53} & -- & \ding{53} & -- & \ding{53} & --\\
10 & 21 & \ding{53} & 295.83 & \ding{53} & -- & \ding{52} & 53.39 & \ding{52} & 3.14 & 10 & 26 & Linear & 1 & \ding{52} & $ 9.40 \pm 7.29 $ & \ding{53} & -- & \ding{108} & --\\
\rowcolor{rowcolor}
11 & 18 & \ding{52} & 77.48 & \ding{53} & -- & \ding{52} & 145.02 & \ding{52} & 3.33 & 11 & 26 & Linear & 1 & \ding{52} & $ 16.82 \pm 16.90 $ & \ding{53} & -- & \ding{53} & --\\
12 & 30 & \ding{52} & 106.137 & \ding{53} & -- & \ding{52} & 71.97 & \ding{52} & 3.37 & 12 & 25 & Linear & 1 & \ding{52} & $ 51.27 \pm 34.43 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
13 & 31 & \ding{52} & 240.24 & \ding{53} & -- & \ding{52} & 39.82 & \ding{52} & 3.07 & 13 & 25 & Linear & 1 & \ding{52} & $ 12.57 \pm 10.57 $ & \ding{53} & -- & \ding{108} & --\\
14 & 18 & \ding{52} & 79.59 & \ding{53} & -- & \ding{52} & 21.9 & \ding{52} & 3.23 & 14 & 29 & Linear & 1 & \ding{52} & $ 19.42 \pm 11.52 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
15 & 20 & \ding{52} & 13.66 & \ding{53} & -- & \ding{52} & 274.79 & \ding{52} & 2.43 & 15 & 37 & Linear & 1 & \ding{52} & $ 58.85 \pm 13.83 $ & \ding{53} & -- & \ding{108} & --\\
16 & 22 & \ding{52} & 30.31 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 6.16 & 16 & 37 & Linear & 1 & \ding{53} & -- & \ding{53} & -- & \ding{108} & --\\
\rowcolor{rowcolor}
17 & 15 & \ding{52} & 24.97 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 2.31 & 17 & 27 & Linear & 1 & \ding{52} & $ 4.80 \pm 3.62 $ & \ding{52} & 66.4 & \ding{53} & --\\
18 & 22 & \ding{52} & 23.7 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 6.47 & 18 & 24 & Linear & 1 & \ding{52} & $ 19.86 \pm 12.17 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
19 & 33 & \ding{52} & 21.41 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 2.47 & 19 & 23 & Linear & 1 & \ding{52} & $ 10.34 \pm 7.59 $ & \ding{53} & -- & \ding{108} & --\\
20 & 22 & \ding{52} & 16.59 & \ding{53} & -- & \ding{52} & 53.57 & \ding{52} & 9.78 & 20 & 25 & Linear & 1 & \ding{53} & -- & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
21 & 21 & \ding{52} & 18.46 & \ding{53} & -- & \ding{52} & 114.8 & \ding{52} & 2.43 & 21 & 24 & Linear & 1 & \ding{52} & $ 12.09 \pm 7.97 $ & \ding{53} & -- & \ding{108} & --\\
22 & 20 & \ding{52} & 18.26 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 9.03 & 22 & 22 & Linear & 1 & \ding{52} & $ 11.79 \pm 11.14 $ & \ding{52} & 29.96 & \ding{108} & --\\
\rowcolor{rowcolor}
23 & 32 & \ding{53} & 108.75 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 2.52 & 23 & 28 & Linear & 1 & \ding{52} & $ 32.71 \pm 24.14 $ & \ding{53} & -- & \ding{53} & --\\
24 & 29 & \ding{53} & 80.94 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 2.38 & 24 & 23 & Linear & 1 & \ding{52} & $ 12.84 \pm 7.20 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
25 & 20 & \ding{52} & 5.43 & \ding{53} & -- & \ding{52} & 16.97 & \ding{52} & 0.2 & 25 & 62 & Linear & 1 & \ding{52} & $ 6.64 \pm 4.62 $ & \ding{53} & -- & \ding{53} & --\\
26 & 33 & \ding{53} & 91.67 & \ding{53} & -- & \ding{53} & -- & \ding{53} & 0 & 26 & 32 & Linear & 1 & \ding{52} & $ 44.89 \pm 49.35 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
27 & 29 & \ding{53} & 86.25 & \ding{53} & -- & \ding{53} & -- & \ding{53} & 0 & 27 & 34 & Linear & 1 & \ding{53} & -- & \ding{53} & -- & \ding{53} & --\\
28 & 21 & \ding{53} & 103.25 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 2.2 & 28 & 26 & Linear & 1 & \ding{52} & $ 11.92 \pm 9.78 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
29 & 25 & \ding{52} & 2.9 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 1.78 & 29 & 35 & Linear & 1 & \ding{52} & $ 16.21 \pm 14.83 $ & \ding{53} & -- & \ding{53} & --\\
30 & 19 & \ding{52} & 3.45 & \ding{53} & -- & \ding{52} & 0.69 & \ding{52} & 0.21 & 30 & 29 & Linear & 1 & \ding{52} & $ 140.51 \pm 67.06 $ & \ding{53} & -- & \ding{108} & --\\
\rowcolor{rowcolor}
31 & 22 & \ding{53} & 67.36 & \ding{53} & -- & \ding{53} & -- & \ding{53} & 0 & 31 & 51 & Multiple & 4 & \ding{53} & -- & \ding{53} & -- & \ding{53} & --\\
32 & 25 & \ding{53} & 27.54 & \ding{53} & -- & \ding{53} & -- & \ding{53} & 0 & 32 & 36 & Multiple & 2 & \ding{52} & $ 71.74 \pm 60.13 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
33 & 20 & \ding{52} & 2.73 & \ding{53} & -- & \ding{52} & 189.06 & \ding{52} & 2.07 & 33 & 27 & Multiple & 2 & \ding{52} & $ 94.02 \pm 58.68 $ & \ding{52} & 26.97 & \ding{53} & --\\
34 & 24 & \ding{52} & 3.47 & \ding{53} & -- & \ding{53} & -- & \ding{52} & 1.34 & 34 & 33 & Multiple & 2 & \ding{52} & $ 57.32 \pm 39.28 $ & \ding{53} & -- & \ding{108} & --\\
\rowcolor{rowcolor}
35 & 22 & \ding{52} & 4.75 & \ding{53} & -- & \ding{52} & 12.04 & \ding{52} & 0.13 & 35 & 27 & Nested & 3 & \ding{52} & $ 58.26 \pm 54.18 $ & \ding{53} & -- & \ding{108} & --\\
36 & 34 & \ding{52} & 4.618 & \ding{53} & -- & \ding{52} & 5.69 & \ding{52} & 0.12 & 36 & 30 & Nested & 2 & \ding{52} & $ 84.23 \pm 57.52 $ & \ding{52} & 17.42 & \ding{53} & --\\
\rowcolor{rowcolor}
37 & 30 & \ding{52} & 6.99 & \ding{53} & -- & \ding{52} & 0.72 & \ding{52} & 0.16 & 37 & 23 & Nested & 2 & \ding{53} & -- & \ding{52} & 0.26 & \ding{108} & --\\
38 & 16 & \ding{52} & 3.43 & \ding{53} & -- & \ding{52} & 0.25 & \ding{52} & 0.27 & 38 & 22 & Nested & 3 & \ding{52} & $ 105.28 \pm 60.01 $ & \ding{53} & -- & \ding{108} & --\\
\rowcolor{rowcolor}
39 & 29 & \ding{52} & 12.94 & \ding{53} & -- & \ding{52} & 0.57 & \ding{52} & 0.16 & 39 & 35 & Nested & 2 & \ding{52} & $ 96.50 \pm 68.99 $ & \ding{53} & -- & \ding{53} & --\\
40 & 18 & \ding{52} & 2.22 & \ding{53} & -- & \ding{52} & 0.84 & \ding{52} & 0.17 & 40 & 26 & Nested & 3 & \ding{52} & $ 139.88 \pm 92.53 $ & \ding{52} & 147.89 & \ding{53} & --\\
\rowcolor{rowcolor}
41 & 23 & \ding{52} & 3.29 & \ding{53} & -- & \ding{52} & 39 & \ding{52} & 0.25 & 41 & 30 & Nested & 2 & \ding{52} & $ 177.43 \pm 106.79 $ & \ding{53} & -- & \ding{53} & -- \\
42 & 21 & \ding{52} & 23.19 & \ding{53} & -- & \ding{52} & 0.67 & \ding{52} & 0.11 & 42 & 29 & Nested & 3 & \ding{52} & $ 228.71 \pm 218.43 $ & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
43 & 24 & \ding{52} & 18.13 & \ding{53} & -- & \ding{52} & 3.14 & \ding{52} & 0.11 & 43 & 39 & Nested & 3 & \ding{53} & -- & \ding{53} & -- & \ding{53} & --\\
44 & 21 & \ding{52} & 4.08 & \ding{53} & -- & \ding{52} & 3.21 & \ding{52} & 0.12 & 44 & 61 & Nested & 4 & \ding{53} & -- & \ding{53} & -- & \ding{53} & --\\
\rowcolor{rowcolor}
45 & 29 & \ding{52} & 34.85 & \ding{53} & -- & \ding{52} & 0.56 & \ding{52} & 0.13 & 45 & 46 & Nested & 3 & \ding{52} & $ 202.78 \pm 185.39 $ & \ding{53} & -- & \ding{53} & --\\
\multicolumn{2}{c|}{} & \multicolumn{8}{c||}{\cellcolor[HTML]{8FBCBB}88 more cases are omitted due to space limitation} & 46 & 24 & Nested & 3 & \ding{52} & $ 86.61 \pm 50.22 $ & \ding{53} & -- & \ding{108} & --\\
\midrule
Total &  & \textbf{114 / 133} &  & 0/133 &  & 73 / 133 & $ 248.01 \pm 982.23 $ & \textbf{124 / 133} & $ 2.1 \pm 2.32$ &  &  &  &  & \textbf{38 / 46} & $ 68.92 \pm 171.13 $  & 9 / 46 & $ 83.03 \pm 104.84 $ & 0 / 46 &\\
\bottomrule
\end{tabular}
}
%\vspace{-15pt}
\end{table*}

==> Table/rq2-svcomp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t!]
\centering
\setlength{\abovecaptionskip}{-0pt}
% \setlength{\belowcaptionskip}{10pt}
\caption{\textbf{Effectiveness on Loop Invariants}. {\footnotesize The benchmark SV-COMP contains 21 C programs with more complex nested/multiple loops.}}
\label{tab:rq2-svcomp}
\scriptsize
\renewcommand\arraystretch{0.8}
    \resizebox{0.9\linewidth}{!}{
\begin{tabular}{l|lrc|cllccr}
\toprule
\multicolumn{4}{c|}{\textbf{Benchmark Information}} & \multicolumn{6}{c}{\cellcolor[HTML]{EBCB8B}\textbf{\name}} \\ \midrule
\textbf{Type} & \textbf{Program} & \textbf{LoC} & \begin{tabular}[c]{@{}l@{}}\textbf{Loop}\\Num.\end{tabular} & \textbf{Success} & \textbf{Ratio} & \textbf{ Iterations} & \begin{tabular}[c]{@{}c@{}}\textbf{Generated}\\ \textbf{Spec}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Correct}\\ \textbf{Spec}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Time(s)}\\ \textbf{mean $\pm$ std}\end{tabular} \\ 
\midrule
\multirow{19}{*}{quantifier-free} & afnp2014\_true-unreach-call.c & 17 & 1 & \ding{52} & 5/5 & 3,1,3,1,1 & 4,4,6,5,4 & 1/1 \iffalse, 3/3\fi  &   $ 40.69 \pm 34.37 $     \\
 & bhmr2007\_true-unreach-call.c & 31 & 1 & \ding{52} & 5/5 & 1,1,1,1,1 & 3,3,4,3,3 & 2/2  &   $ 4.50 \pm 2.61 $        \\
 & cggmp2005\_true-unreach-call.c & 18 & 1 & \ding{52} & 1/5 & 5,5,4,5,5 & 4,5,4,4,4 & 3/3 &   $ 128.04 \pm 53.74 $        \\
 & count\_up\_down\_true-unreach-call\_true-termination.c & 22 & 1 & \ding{52} & 5/5 & 1,1,1,1,1 & 5,4,5,6,5 & 2/2 &   $ 18.44 \pm 15.77 $     \\
 & css2003\_true-unreach-call.c & 19 & 1 & \ding{52} & 4/5 & 1,-,1,1,1 & 8,8,8,5,11 & 3/3  &   $ 88.07 \pm 74.35 $     \\
 & ddlm2013\_true-unreach-call.c & 33 & 1 & \ding{53} & 0/5 & -,-,-,-,- & 8,20,13,30,13 & 0/1  &   --        \\
 & down\_true-unreach-call.c & 21 & 2 & \ding{52} & 3/5 & -,1,-,5,1 & 21,12,22,40,24 & 3/3 &   $ 269.98 \pm 224.05 $       \\
 & half\_2\_true-unreach-call.c & 25 & 2 & \ding{53} & 0/5 & -,-,-,-,- & 44,17,12,18,32 & 0/2  &   --        \\
 & hhk2008\_true-unreach-call.c & 26 & 1 & \ding{52} & 5/5 & 1,1,1,1,1 & 4,5,4,5,5 & 2/2   &   $ 8.49 \pm 5.87 $       \\
 & jm2006\_variant\_true-unreach-call.c & 30 & 1 & \ding{52} & 5/5 & 1,1,1,1,1 & 6,8,10,6,8 & 2/2  &   $ 22.52 \pm 14.55 $     \\
 & jm2006\_true-unreach-call.c & 25 & 1 & \ding{52} & 1/5 & 5,1,5,5,5 & 3,4,3,6,4 & 0/1    &   $ 123.61 \pm 100.31 $       \\
 & large\_const\_true-unreach-call.c & 37 & 2 & \ding{53} & 0/5 & -,-,-,-,- & 88,69,40,82,31 & 1/3    &   --        \\
 & nest-if3\_true-unreach-call.c & 19 & 2 & \ding{52} & 5/5 & 2,1,1,1,1 & 8,7,10,9,8 & 3/3 &   $ 107.05 \pm 73.11 $        \\
 & nested6\_true-unreach-call.c & 31 & 3 & \ding{53} & 0/5 & -,-,-,-,- & 74,48,63,43,52 & 2/4    &   --     \\
 & nested9\_true-unreach-call.c & 23 & 3 & \ding{52} & 5/5 & 1,1,1,1,1 & 25,23,28,22,25 & 4/4  &   $ 274.87 \pm 156.77 $       \\
 & seq\_true-unreach-call.c & 33 & 3 & \ding{53} & 0/5 & -,-,-,-,- & 52,16,50,17,28 & 4/5    &   --       \\
 & sum01\_true-unreach-call\_true-termination.c & 20 & 1 & \ding{52} & 5/5 & 1,1,1,1,1 & 6,8,6,8,6 & 2/2   &   $ 8.12 \pm 6.41 $       \\
 & terminator\_03\_true-unreach-call\_true-termination.c & 20 & 1 & \ding{52} & 5/5 & 1,1,1,1,1 & 2,2,2,3,2 & 1/1  &   $ 26.09 \pm 22.98 $     \\
 & up\_true-unreach-call.c & 30 & 2 & \ding{52} & 3/5 & 5,2,2,-,- & 27,14,10,28,0 & 3/3    &   $ 374.38 \pm 291.44 $       \\ \hline
\multirow{2}{*}{quantifier} & array\_true-unreach-call1 & 13 & 1 & \ding{52} & 5/5 & 1,1,1,1,1 & 4,3,3,3,3 & 1/1  &   $ 5.88 \pm 3.78 $       \\
 & array\_true-unreach-call2 & 18 & 1 & \ding{52} & 5/5 & 1,1,1,1,1 & 4,4,5,4,4 & 1/1  &   $ 32.53 \pm 27.11 $     \\
 \midrule 
 \textbf{Total} & & & &  \textbf{16 / 21} & & & & & \textbf{$217.85$} $\pm 451.72 $\\
 \bottomrule
 
\end{tabular}
}
\vspace{-0.5pt}
\end{table*}

==> Tex/051-implementation.tex <==
\framac (Framework for modular analysis of C programs)~\cite{kirchner2015frama,beyer2022static} is an extensible and collaborative platform dedicated to source-code analysis. It is mainly co-developed at the Software Security and Reliability Laboratory of CEA-LIST and the Toccata team of INRIA Saclay.

The \wpplugin plugin in \framac implements deductive verification calculus, a modular sound technique to prove that a property holds after the execution of a function if some other properties hold before it (pre/post condition as seen before).
\wpplugin is able to verify more complex logical annotations and assertions using external automated or interactive provers (mainly AltErgo, Why3 and Coq) but requires extra efforts with the code annotations, including loop annotations. Indeed, to analyze a source code with loops, WP needs a specification for each of them, or it uses an implicit specification, which is equivalent to "anything can happen".

\textbf{Theorem Provers}. The VCs generated by WP can be submitted to an interactive or automatic theorem prover. Frama-C natively supports two provers: the
Alt-Ergo automatic prover and the Coq proof assistant. Other provers are supported through the Why platform1. In the experiments reported in this paper
the following provers were used:
– Alt-ergo 0.95.1
– Z3 4.3.1 (through the Why platform)
